A Higgs Boson at 96 GeV?!

We briefly summarize some searches for Higgs bosons with a mass of m_phi <= 110 GeV at LEP and the LHC. We discuss a possible signal in the diphoton decay mode at m_phi = 96 GeV as reported by CMS, together with a 2 sigma hint in the bb final state at LEP. We briefly review possible interpretation of such a new particle in various BSM models. We focus on possible explanations as reported within the NMSSM and the munuSSM. Conclusions for future collider projects are briefly outlined.

==> preprint.tex <==
IFT--UAM/CSIC--18-125\\
DESY 18-221
%arXiv:1411.6526 [hep-ph]

